Real-Time Diagnostic Integrity Meets Efficiency: A Novel Platform-Agnostic Architecture for Physiological Signal Compression

Head-based signals such as EEG, EMG, EOG, and ECG collected by wearable systems will play a pivotal role in clinical diagnosis, monitoring, and treatment of important brain disorder diseases. However, the real-time transmission of the significant corpus physiological signals over extended periods consumes substantial power and time, limiting the viability of battery-dependent physiological monitoring wearables. This paper presents a novel deep-learning framework employing a variational autoencoder (VAE) for physiological signal compression to reduce wearables' computational complexity and energy consumption. Our approach achieves an impressive compression ratio of 1:293 specifically for spectrogram data, surpassing state-of-the-art compression techniques such as JPEG2000, H.264, Direct Cosine Transform (DCT), and Huffman Encoding, which do not excel in handling physiological signals. We validate the efficacy of the compressed algorithms using collected physiological signals from real patients in the Hospital and deploy the solution on commonly used embedded AI chips (i.e., ARM Cortex V8 and Jetson Nano). The proposed framework achieves a 91% seizure detection accuracy using XGBoost, confirming the approach's reliability, practicality, and scalability.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In our research paper, we introduced an innovative approach for compressing physiological signals with an exceptional compression ratio (1:293), outperforming all existing methods. Furthermore, we assessed the effectiveness of our compression by inputting the compressed signals into a classifier for detecting seizures. Remarkably, we achieved comparable accuracy (91\%) compared to using the original uncompressed signals (98\%). In the hardware implementation phase, we successfully deployed our model on various chips such as Jetson Nano and Raspberry Pi. We observed energy efficiency improvements when utilizing the compressed signals, leading to power savings in contrast to using the original uncompressed signals. Despite achieving an impressive compression ratio compared to earlier efforts and maintaining comparable accuracy, there remains ample potential to further enhance signal compression beyond current achievements. This could potentially lead to reaching accuracy level when utilizing the original uncompressed signals. Also, we can improve inference time too because it is not completely a real time application.
